Flover: A Temporal Fusion Framework for Efficient Autoregressive Model Parallel Inference

Autoregressive models, despite their commendable performance in a myriad of generative tasks, face challenges stemming from their inherently sequential structure. Inference on these models, by design, harnesses a temporal dependency, where the current token's probability distribution is conditioned on preceding tokens. This inherent characteristic severely impedes computational efficiency during inference as a typical inference request can require more than thousands of tokens, where generating each token requires a load of entire model weights, making the inference more memory-bound. The large overhead becomes profound in real deployment where requests arrive randomly, necessitating various generation lengths. Existing solutions, such as dynamic batching and concurrent instances, introduce significant response delays and bandwidth contention, falling short of achieving optimal latency and throughput. To address these shortcomings, we propose Flover -- a temporal fusion framework for efficiently inferring multiple requests in parallel. We deconstruct the general generation pipeline into pre-processing and token generation, and equip the framework with a dedicated work scheduler for fusing the generation process temporally across all requests. By orchestrating the token-level parallelism, Flover exhibits optimal hardware efficiency and significantly spares the system resources. By further employing a fast buffer reordering algorithm that allows memory eviction of finished tasks, it brings over 11x inference speedup on GPT and 16x on LLAMA compared to the cutting-edge solutions provided by NVIDIA FasterTransformer. Crucially, by leveraging the advanced tensor parallel technique, Flover proves efficacious across diverse computational landscapes, from single-GPU setups to distributed scenarios, thereby offering robust performance optimization that adapts to variable use cases.

==> inception.tex <==
\vspace{-1em}
\begin{figure}[h]\centering
    \includegraphics[width=0.8\linewidth]{figures/inception.png}
    % \caption{Subfigure 1}
    % \label{fig:subfigure1}
    % \vspace{-1em}
\caption{Using NVIDIA Triton Perf\_analyzer to evaluate the efficiency of concurrent model instances, where per request uses a dedicated model instance. Blue line denotes the ideal latency with no overhead. \textcolor{red}{will replace this figure}}
\label{fig:inception}
\end{figure}

==> memory_fusion.tex <==
\begin{figure}[t]\centering
\includegraphics[width=1.0\linewidth]{memory_fusion_.pdf}
\caption{Illustration on how request fusion works on the memory level. We make sure that tensors of different requests are located adjacent to each other, forming a contiguous memory space.}
\vspace{-1em}
\label{fig:memory_fusion}
\end{figure}

==> memory_shuffle2.tex <==
\begin{figure}[t]\centering
 % \vspace{-1em}
\includegraphics[width=1.0\linewidth]{shufflea.drawio.pdf}
\vspace{-1em}
\caption{Array in (a) represents the GPU memory space. $1$ denotes the memory region of currently running requests; (b) shows the optimal memory shuffle strategy given the layout, where we only need to move 3 pieces of memory to form a new contiguous memory region.}
\vspace{-1em}
\label{fig:memory_shuffle2}
\end{figure}

==> poisson2.tex <==
\begin{table}
\setlength{\tabcolsep}{4.2pt}
    \begin{tabular}{c|c| c | c |c |c|c|c}
    \toprule[2pt]
     $\lambda$ (ms) & 20 & 50 & 100 & 150 & 200 & 300 & 400  \\
    \toprule[1pt]
    
    Overlap & 91.3\% & 81.8\% & 67.3\% & 62.1\% & 60.3\% & 45.2\% & 36.7\%\\
    \hline
     Speedup & 11.2x & 11.1x & 10.2x & 9.3x & 9.1x & 7.9x & 7.1x\\
    \hline
    Total Iters. & 557 & 616  &  748 & 888 & 911 & 1174 & 1366\\
    \hline
    
    \toprule[2pt]
    $\lambda$ (ms) &  500 & 750 & 1000 & 2000 & 3000 & 4000 & 5000 \\
    \toprule[1pt]
    
    Overlap & 31.0\% & 23.2\% & 20.0\% & 9.3\% & 6.7\% & 5.7\% & 4.8\%\\
    \hline
     Speedup &  6.5x & 4.5x & 4.2x & 2.1x & 1.3x & 1.3x & 1.1x \\
    \hline
    Total Iters. & 1537 & 2239 & 2621 & 5483 & 7738 & 8902 & 10694 \\
    \hline
    \toprule[2pt]
    \end{tabular}
    \caption{Comparison on number of temporally overlapped requests, speedup to FasterTransformer, and total iterations for inferring 32 requests follow the Poisson process of different $\lambda$. Single request require 504 iterations to generate all output tokens.
    }
    \label{tab:poisson2}
    % \vspace{-1em}
\end{table}

==> shuffle2.tex <==
\begin{figure}[h]\centering
    \includegraphics[width=\linewidth]{shuffle_res_.pdf}
    % \caption{Subfigure 1}
    % \label{fig:subfigure1}
    \vspace{-1em}
\caption{Total latency of inferring 32 requests with random number of iterations. Time intervals between requests are fixed at 20ms. \texttt{128-256} denotes every request's total iterations follows a uniform distribution with lower bound at 128 and upper bound at 256.}
\label{fig:shuffle1}
\end{figure}

==> shuffle_res.tex <==
\begin{figure}[h]\centering
    \includegraphics[width=\linewidth]{shuffle_res_.pdf}
    % \caption{Subfigure 1}
    % \label{fig:subfigure1}
    \vspace{-1em}
\caption{Total latency of inferring 32 requests with random number of iterations. Time intervals between requests are fixed at 20ms. \texttt{128-256} denotes every request's total iterations follows a uniform distribution with lower bound at 128 and upper bound at 256.}
\label{fig:shuffle_res}
\end{figure}

==> x2-related_work.tex <==
\section{Background}
\textcolor{red}{This is background, not related work.}
\paragraph{\textbf{Autoregressive models}} Deep learning architectures encompass a diverse array of models, each with its unique characteristics and applicability. Predominantly, these models can be broadly categorized into non-autoregressive and autoregressive types, distinguished by their distinct operational mechanisms.

\textcolor{red}{This subsection is called autoregressive models, but you are comparing and contrasting both types. Maybe you can rename it to Non-autoregressive vs Autoregressive Neural Networks.}
Non-autoregressive models, such as ResNet for image classification and YOLO for object detection, are extensively employed in a variety of applications. The essence of these models lies in their feed-forward design. This design implies that an input undergoes a series of transformations to produce an output, independent of other inputs. Models such as ResNet and YOLO are emblematic of this category. ResNet, a convolutional neural network, processes an image through multiple layers to output class probabilities. Similarly, YOLO, utilized for object detection tasks, predicts bounding boxes and associated class probabilities for detected objects in an input image. The absence of temporal dependencies within these models means that each input is processed autonomously, without requiring retention or reference to any preceding input.

In contrast, autoregressive models constitute a distinct class of deep learning models, differentiated by their inherent temporal dependencies. Unlike their non-autoregressive counterparts, the output at each step within these models is influenced by the preceding steps. This trait makes them particularly suitable for tasks such as natural language processing and time series analysis, where the sequential order of data points is of paramount importance. However, the sequential nature of these models introduces unique challenges pertaining to latency and computational resource utilization during inference, which are the primary focus of this work.

\paragraph{\textbf{Model inference}} Traditionally, the bulk of the research in the deep learning community has been focused on the training phase. This is largely due to the complexity and computational intensity of training large-scale models, however, with the advent of large language models (LLMs) and other sophisticated architectures, there is an increasing recognition of the importance of efficient inference. Deep learning model inference, particularly in production environments, 

requires careful management of resources and latency. Inference frameworks, such as NVIDIA's Triton Inference Server or Microsoft's ONNX Runtime, play a critical role in this regard. These frameworks provide a suite of tools for deploying models, managing computational resources, handling multiple requests concurrently, and optimizing performance. They are specifically designed to ensure that the inference process is as efficient and scalable as possible.


Efforts to enhance deep learning model inference have manifested in a variety of techniques aimed at optimizing computational efficiency, reducing memory usage, and decreasing latency. These techniques include quantization, which reduces numerical precision of model weights and activations; mixed precision computations, which combine different numerical precisions to balance computational speed and numerical accuracy; kernel fusion, which consolidates multiple layers or operations into a single computational kernel to minimize overhead; and zero offload, a strategy devised to handle large models by offloading parts of the model's weights and optimizer states to CPU memory. While these techniques have significantly advanced model inference, they do not inherently consider or exploit the temporal dependencies that are intrinsic to autoregressive models. This oversight can lead to limited efficiency in the inference phase of these models, as the potential benefits derived from understanding and leveraging the temporal nature of autoregressive tasks are not realized. This gap in the current landscape of model inference techniques underscores the need for strategies that are specifically designed with the peculiarities of autoregressive models in mind, a challenge that this paper aims to address.

